Higgs Working Group Summary Report

Report of the Working Group on Higgs Bosons for the Workshop, ``Physics at TeV Colliders'', Les Houches, France, 11-29 June, 2007.

==> cpvhiggs.tex <==
%\documentclass[11pt]{cernrep}
%\usepackage{graphicx,epsfig}
%\usepackage{cite}
%\bibliographystyle{lesHouches}
%\begin{document}
%\title{Search for the $t \to bH^{+}$, $H^{+} \to H_{1}W$, $H_{1}\to b\bar{b}$
%       channel in CPX MSSM scenario in CMS
%       ~\footnote{results are preliminary and must not be shown 
%         on the conferences}}
%\author{A. K. Nayak$^1$, T. Aziz$^1$, A. Nikitenko$^2$}
%\institute{$^1$Tata Institute of Fundamental Research, Mumbai,India \\
%$^2$ Imperial College, London, on leave from ITEP, Moscow, Russia}
%\maketitle
%%\begin{abstract}
%\end{abstract}

\section{Introduction}

CP violation (CPX) in the Higgs sector of the Minimal Supersymmetric Standard Model (MSSM), 
when the Higgsino mass parameter $\mu$, the gaugino mass parameters $M_{i}$ and 
the trilinear couplings $A_{f}$ are complex, allows the existence of the light neutral Higgs boson
($m_{H_{1}} \leq$ 50 GeV) and relatively light charged Higgs boson 
($m_{H^{+}} \le m_{t}$) in low tan$\beta$ region not excluded by the LEP 
data because of the reduction of $H_{1}ZZ$ coupling \cite{Schael:2006cr}. 
In CPX scenario the usual search channels may not be useful, because 
of the simultaneous reduction in the couplings of the Higgs boson to the vector 
boson pair and to the top quark pair, as it affects the Higgs boson 
production and decays rates. The one of the promising search channels in 
the CPX scenario proposed in \cite{Ghosh:2004cc} is the $t \bar{t}$ production 
when one of the top quarks decays as 
$t \to bH^{+}$, $H^{+} \to H_{1}W$, $H_{1}\to b\bar{b}$. It is due to
the suppression of the $H_{1}ZZ$ coupling leads to the enhancement of the 
$H^{+}W^{-}H_{1}$ coupling in order to satisfy the coupling sum-rule. 
We investigated a feasibility for the discovery of the Higgs bosons in 
this channel using the full CMS detector simulated data. The results
shown are preliminary.

\section{Event generation}

The signal events were generated using PYTHIA \cite{Sjostrand:2006za} 
with $m_{t}$=175 GeV, $m_{H_{1}}$=51 GeV and $m_{H^{+}}$=133 GeV, 
corresponding to tan$\beta$=5 and CP mixing angle $\Phi$(CP)=$90^0$ in 
the CPX MSSM. The following decays were forced in PYTHIA:
$t_{1} \to bW$, $t_{2} \to bH^{+}$, $H^{+} \to WH_{1}$, $H_{1} \to b\bar{b}$ 
and both $W$ bosons from the top decays were allowed to decay into all possible 
modes. The decay branching fractions were calculated using CPsuperH 
program~\cite{Lee:2003nta}. The total cross section was calculated taking 
the next-to-leading order cross section for an inclusive $t\bar{t}$ 
production 840 pb ~\cite{Beneke:2000hk} and multiplying by the branching 
ratios, Br($t \to bH^{+}$)=0.01, Br($H^{+} \to H_{1}W$)=0.567, 
Br($t \to bW$)=0.99, Br($H_{1} \to b \bar{b}$)=0.92 which gives the 
cross section 8.68 pb.

The major background processes for this channel are  $t\bar{t} + \rm jets$ 
and $t\bar{t}b\bar{b}$. The $t\bar{t} + \rm jets$ background  
was generated using ALPGEN~\cite{Mangano:2002ea} with the MLM prescription 
for jet-parton matching~\cite{Mangano:2006rw,Hoche:2006ph} at the PYTHIA 
shower simulation. The $t \bar{t}+\rm 2~jets$ (exclusive), 
$t \bar{t}+\rm 3~jets$ and $t \bar{t}+\rm 4~jets$(inclusive) with 
jet $p_{T}>$20 GeV were generated. The cross sections for these processes 
are shown in Table~\ref{table1}.  The $t\bar{t}b\bar{b}$ background was not 
considered yet in this study.

\section{Simulation and Reconstruction}

The CMS detector was simulated using full GEANT4 \cite{Agostinelli:2002hh} 
simulation and the reconstruction was done using the CMS simulation and 
reconstruction software CMSSW. No pileup events were included. We summarize
briefly the object reconstruction methods~\cite{ptdr1:2006cms} used in this 
analysis. Muons are reconstructed from the muon chambers and the silicon tracker and 
electrons are reconstructed from the tracks in the silicon tracker and the
clusters in the electromagnetic calorimeter. The loose electron identification 
criteria were applied. The lepton isolation was done using the tracker isolation such 
that leptons are selected if sum $p_{T}$ of the tracks in a cone around the lepton 
(inner radius 0.015 and outer radius 0.25) is less than 3 GeV.  The jets were 
reconstructed from the calorimeter towers using an iterative cone algorithm with the
cone size 0.5. The jet energy was corrected using the Monte Carlo jet energy corrections. 
The missing $E_{T}$ was reconstructed from the calorimeter towers and corrected for the 
jet energy scale. The missing $E_{T}$ was also corrected for the muons by adding the muon 
momenta to the calorimeter missing $E_{T}$.

\section{Event selection}

\subsection{Primary selections}

The final state considered in this analysis consists of two light quarks, four b quarks,
one lepton and neutrino: $\ell\nu+qq'+b\bar{b}b\bar{b}$. Since the neutral Higgs boson $H_{1}$ is very light 
(51 GeV), the b quarks from the $H_{1} \to b \bar{b}$ decay are very soft as seen in 
Fig.\ref{cpvh1} (a,b). Only $\simeq 36\%$ of events have both b quarks from the $H_{1}$ decay 
with $p_{T}^{b}>$20 GeV. The final state quarks in the event fall very close to each other 
in ($\eta, \phi$) space.  Fig.~\ref{cpvh1} (c) shows the separation in ($\eta, \phi$) space 
between two closest quarks. Because of these reasons it is difficult to reconstruct six jets 
in the event corresponding to the six final states quarks.
\begin{figure}[htbp]
\begin{center}
\includegraphics[width = 5cm, height = 5cm]{PtOfAllbQuarks.eps}\includegraphics[width = 5cm, height = 5cm]{PtOfbQuarksFromH1.eps}\includegraphics[width = 5cm, height = 5cm]{Separation_closestQuarks.eps}
$\mbox{(a)} \hspace{4.5cm}  \mbox{(b)} \hspace{4.5cm} \mbox{(c)}$
\caption{(a) $p_{T}$ distribution of b quarks from top quark and from $H_{1}$ decays, 
         (b) $p_{T}$ distribution of b quarks from $H_{1}$ decay, 
         (c) the $\Delta R$ separation in ($\eta, \phi$) space between two closest final state 
             quarks in the event.}
\label{cpvh1}
\end{center}
\end{figure}
The events with one isolated lepton with $p_{T}>$20 GeV and six or more jets with $E_{T}>$20 GeV
were selected.  The number of leptons in the event (electrons with $p_{T}>$ 10 GeV and
muons with $p_{T}>$5 GeV) passing the identification and the isolation were counted and
the events with more than one lepton were rejected. The jets were b tagged using the track counting 
b-tagging algorithm. The three dimensional impact parameter significance of the second highest 
significance track in the jet was used as the b-discriminator parameter. The four highest 
discriminator jets with the discriminator value greater than 2.95 were tagged as b jets. 

\subsection{Top mass reconstruction}

One $W$ boson in the event was reconstructed from the lepton and the missing $E_{T}$. 
The z-component of the missing energy was calculated using the $W$ mass constraint. 
This yields the real solutions in nearly 66\% events. The events with the imaginary solutions 
were rejected. There are two possible solutions for the z-component of the missing energy which gives 
two possible candidates for the leptonically decaying $W$ boson. The $W$ boson decaying hadronically 
was reconstructed from the jets not tagged as b jets. All jet pairs with the invariant mass within 
the $m_{W}\pm$ 20 GeV mass window were considered as possible candidates. 
The di-jets invariant mass for the jets matching to quarks from the $W$ boson decay is shown in 
Fig.\ref{cpvh2} (a). 
\begin{figure}[h!]
\begin{center}
\includegraphics[width = 5cm, height = 5cm]{IdealWFromTop.eps}
\includegraphics[width = 5cm, height = 5cm]{RecoTopbjjSignal.eps}
\includegraphics[width = 5cm, height = 5cm]{RecoTop3bjjSignal.eps} \\
$\mbox{(a)} \hspace{4.5cm}  \mbox{(b)}\hspace{4.5cm}  \mbox{(c)}$
\caption{(a) the di-jet invariant mass of the jets matching to quarks from $W$ decay. 
         (b) the top-quark mass reconstructed from the bjj final state after the minimization of $\delta M$.
         (c) the top-quark mass reconstructed from bbbjj final state after the minimization of $\delta M$.}
\label{cpvh2}
\end{center}
\end{figure}
The momenta of the two top quarks were reconstructed simultaneously from four b-tagged jets, 
two $W \to \ell \nu$ candidates and candidates for the hadronically decaying $W$ boson. 
The jets and the $W$ boson candidates were assigned to the two top quarks by minimizing the $\delta$M, 
where $\delta$M is defined as
\begin{eqnarray}
\delta \rm M = \sqrt{(m_{top1} - m_{top})^{2} + (m_{top2} - m_{top})^{2} +(m_{W(hadronic)} - m_{W})^{2}},   
\end{eqnarray}
there $m_{top1}$ is reconstructed from one b-tagged jet and one $W$ boson candidate, 
$m_{top2}$ is reconstructed from three b-tagged jets and one $W$ boson candidate, $m_{top}$ is the
generated top-quark mass (175 GeV) and the $m_{W}$ is the $W$ boson mass (PDG value). 

The top-quark mass distributions reconstructed from three jets ($bjj$)
and five jets ($bbbjj$) after the minimization of $\delta M$ are shown in Fig.\ref{cpvh2} (b,c). 
One can see that the top-quark mass distribution from the $bbbjj$ final state is very wide and has 
a big tail. It is because of wrong assignment of the jets or $W$ candidates to the top while 
minimizing $\delta M$. The events with the two top-quark reconstructed masses within the $m_{top} \pm$ 30 GeV 
mass window were selected. Table~\ref{table1} shows the initial cross sections for the signal and 
background processes, the number of Monte-Carlo events remaining after each selection step and 
the cross sections after all selections. 
~\footnote{the $W \to \ell \nu$ and $W \to \rm jj$ reconstruction step selects events with the positive solution 
           for z-component of $E_{T}^{miss}$ and with at least one jet pair having the di-jet mass within 
           the $m_{W}\pm$ 20 GeV mass window; the top-quark mass reconstruction step requires that the two top-quark 
           reconstructed masses are within the $m_{top} \pm$ 30 GeV mass window.}
\begin{table}
\caption{The initial cross sections for the signal and background processes, 
         the number of Monte Carlo events remaining after each selection steps and 
         the cross section after all selections.}
\label{table1}
\begin{center}
\begin{tabular*}{0.95\textwidth}{@{\extracolsep{\fill}}|c|c|c|c|c|}\hline
   & signal & $t \bar{t}+\rm 2~jets$ & $t \bar{t}+\rm 3~jets$ & $t \bar{t}+\rm 4~jets$ \\
   &        &(exclusive)&(exclusive)&(inclusive)\\
\hline
\hline
cross section, pb                        & 8.68    &    100 &     40  &     61  \\
\hline
\hline
number of MC events analyzed             & 193884  & 241000 &  71000  &  94000  \\
(corresponding luminosity, fb$^{-1}$)    & (22.35) & (2.41) & (1.775) & (1.54)  \\
\hline
isolated lepton $p_{T}>$ 20 GeV          & 41035   & 57920  &   16915 &  22214  \\
\hline
$\geq$ 6 jets $E_{T}>$ 20 GeV              & 21389   & 36315  &   14479 &  21866  \\
\hline
4 b-tagged jets with discr. $>$2.95      &   881   &   371  &     248 &   1069  \\
\hline
$W \to \ell \nu$ and $W \to \rm jj$ reco &   379   &   158  &     132 &    602  \\
\hline
top-quark mass reconstruction            &    83   &     4  &       1 &      7  \\
\hline
\hline
cross section after all selections, fb   &   3.71  &   1.66 &    0.56 &   4.54 \\
\hline
\end{tabular*}
\end{center}
\end{table}

\subsection{Reconstruction of the neutral $H_{1}$ and charged $H^{+}$ Higgs bosons}

Since it is not known what pair of the b-tagged jets from the reconstructed top quark decay 
chain $t \to bbbW$ is coming from the $H_{1} \to b \bar{b}$ decay, all three b-tagged jet 
pairs were considered as the possible candidates. The invariant mass of b-tagged jet pairs, 
$m_{bb}$ is shown in Fig.~\ref{cpvh3} (left plot) for the background and the signal plus background.
The right plot in Fig.~\ref{cpvh3} shows, fitted by the Gaussian the $m_{bb}$ distribution of the 
signal plus background. The mean value of the fitted distribution is close to the generated mass of 
$H_{1}$. The charged Higgs boson was reconstructed from the two b-tagged jets and $W$ boson, where the 
b-tagged jet pair was chosen as the jet pair with the invariant mass closest to the peak of the $m_{bb}$ 
mass distribution and within the window $\pm$20 GeV around the fitted mean value. 
The invariant mass distribution of the charged Higgs boson reconstructed in this way, $m_{bbW}$ is 
shown in Fig.\ref{cpvh4}.
\begin{figure}[h!]
\begin{center}
\includegraphics[width = 6cm, height = 6cm]{RecoH1Mass.eps}
\includegraphics[width = 6cm, height = 6cm]{RecoH1MassFitted.eps} 
\caption{The invariant mass of the b-tagged jet pairs from the reconstructed top quark decay chain $t \to bbbW$}
\label{cpvh3}
\end{center}
\end{figure}
\begin{figure}[h!]
\begin{center}
\includegraphics[width = 6cm, height = 6cm]{RecoHplusMass.eps}
%\includegraphics[width = 6cm, height = 6cm]{RecoHplusMassFitted.eps}
\caption{The invariant mass of two b-tagged jets and $W$ boson, where two b-tagged jets were chosen
         with the mass closest to the peak of the $m_{bb}$ mass distribution and within the window 
         $\pm$20 GeV around the fitted mean value }
\label{cpvh4}
\end{center}
\end{figure}

The available Monte Carlo statistics of $t \bar{t}+ \rm jets$ background events for this study 
was only order of $\simeq$ 2 fb$^{-1}$, thus it can not be simply rescaled in order to produce the
smooth shape of $m_{bb}$ and $m_{bbW}$ distributions expected for 30 fb$^{-1}$ after all selections. 
We have obtained, however that the shape of $m_{bb}$ and $m_{bbW}$ distributions is almost the same 
after relaxing the cut on the b-discriminator value. Fig.~\ref{cpvh5} shows the $m_{bb}$ (left plot) and 
$m_{bbW}$ (right plot) distributions for four different b-discriminator cuts: 0, 1.0, 1.5 and 2.0. 
\begin{figure}[h!]
\begin{center}
\includegraphics[width = 6cm, height = 6cm]{RecoH1MassBkg.eps}
\includegraphics[width = 6cm, height = 6cm]{RecoHplusMassBkg.eps}
\caption{The $m_{bb}$ (left) and $m_{bbW}$ (right) distributions after all selections for four different
         cuts on the b-discriminator value: 0, 1.0, 1.5 and 2.0.}
\label{cpvh5}
\end{center}
\end{figure}

\section{Results}

The simple selection strategy described in the 
previous sections yields S=110 signal events and B=203 $t\bar{t}+ \rm jets$ 
background events expected with 30 fb$^{-1}$.
The $t\bar{t}b\bar{b}$ background still need to be taken into account. 
The uncertainty due to the Monte Carlo statistics on the $t \bar{t}+ \rm jets$ 
backgrounds is $\simeq$ 30$\%$. The experimental systematic uncertainty was 
estimated by taking into account the systematic uncertainties on the lepton 
identification (2$\%$), the b-jet tagging (5$\%$ per jet), the jet energy 
scale (5$\%$ per jet), the missing transeverse energy scale (10$\%$ on the
raw calorimeter energy scale and 5$\%$ on the jet energy scale) and the 
luminosity uncertainty (5$\%$). It leads to the total systematic uncertainty 
22.5$\%$ (the uncertainty due to the jet and the missing $E_{T}$ scale only 
is 8.8\%).  The significance is calculated as $S/\sqrt{B+ \Delta{B}^{2}}$, 
where $\Delta{B}$ is the experimental systematic uncertainty on the background. 
In order to get the pessimistic value for the significance, the Monte Carlo statistical 
uncertainty was added to the total background: B=203+60=263 events. The signal significance 
is then 110/$\sqrt{263+59^{2}}$=1.8. The uncertainty on the theoretical leading-order cross 
section of the $t \bar{t} + \rm n~jets$, (n$\geq$2) processes is $\geq$50\%. 

One can see that the discovery potential is restricted by both the experimental and the
theoretical uncertainties. The uncertainties can be partially
reduced if the number of the background events and the $m_{bb}$ and $m_{bbW}$ mass shapes
can be extracted from the data. The shapes can be evaluated from the data with the ratio 
S/B$<<$1 when the relaxed cut on the b-discriminator value is used (see Fig.~\ref{cpvh5}). The background 
normalization on the number of events with the relaxed b-jet tagging will eliminate the jet and the  
missing $E_{T}$ scale uncertainties, the luminosity uncertainty and partially reduce the b-tagging 
uncertainty which dominates the experimental uncertainty. It will also reduce the
absolute background prediction uncertainty from the theory, since only the ratio of
$t \bar{t} + \rm jets$ and $t \bar{t} b \bar{b}$ cross sections need to be used. The further, 
more detailed investigations of this channel is foreseen in CMS. 

%expected no. of events for 30 fb^-1
%                        tt~         signal
%B-discriminator > 0.    5716         746  shape of bkg from data
%B-discriminator > 1.0   4477         665
%B-discriminator > 1.5   2455         456
%B-discriminator > 2.0   1110         280

\section*{ACKNOWLEDGEMENTS}

We would like to thank R.~Godbole for very useful discussions and providing the
code calculating Br($t \to bH^{+}$). We would like to thank our CMS colleagues
Joanne Cole and Claire Shepherd-Themistocleous for the discussions about the optimal
strategy for the jet reconstruction and assignment. Finally A.K.N. and A.N. thank 
organizers of Les Houches Workshop 2007 for the warm hospitality and the friendly 
and stimulating atmosphere.

\bibliography{cpvhiggs}

\end{document}



==> hnnlolh.tex <==
%\documentclass[11pt]{cernrep}
%\usepackage{graphicx,epsfig}
%\bibliographystyle{lesHouches}
\def\ptmin{p_{T{\rm min}}}
\def\ptmax{p_{T{\rm max}}}
\newcommand\as{\alpha_{\mathrm{S}}} 
%\begin{document}


%\title{HNNLO: a Monte Carlo program for Higgs boson production at the LHC}

%\author{S.~Catani, M.~Grazzini}
%\institute{INFN, Sezione di Firenze, Via Sansone 1, I-50019 Sesto Fiorentino, Florence, Italy}
%
%\maketitle
%
%\begin{abstract}
%We consider Higgs boson production through gluon--gluon fusion in hadron collisions. We present a numerical program that computes the cross section up to NNLO in QCD perturbation theory. The program includes the decay modes $H\to\gamma\gamma$ and $H\to WW\to l\nu l\nu$,
%and allows the user to apply arbitrary cuts on the momenta of
%the partons and
%of the leptons (photons) produced in the final state.
%\end{abstract}

%\section{INTRODUCTION}
\subsection{Introduction}

Gluon-gluon fusion is the main production channel of
the Standard Model Higgs boson at the LHC.
At leading order (LO) in QCD perturbation theory, the cross section is proportional
to $\as^2$, $\as$ being the QCD coupling. The QCD radiative corrections to the total cross section are known at the
next-to-leading order (NLO) 
\cite{Dawson:1990zj,Djouadi:1991tka,Spira:1995rr}
and at the next-to-next-to-leading order (NNLO) 
\cite{Harlander:2000mg,Catani:2001ic,Harlander:2001is,Harlander:2002wh,Anastasiou:2002yz,Ravindran:2003um}.
The effects of a jet veto on the total cross section has been studied
up to NNLO \cite{Catani:2001cr}.
We recall that all the results at NNLO have been obtained by using 
the large-$M_t$ approximation, $M_t$ being the mass of the top quark.

These NNLO calculations are certainly important but they refer
to situations where the experimental cuts
are either ignored (as in the case of the total cross section) or taken into account
only in simplified cases (as in the case of the jet vetoed cross section).
The impact of higher-order corrections
may be strongly dependent on the details of the applied cuts and also the shape of the
distributions is typically affected by these details.

The first NNLO calculation that fully takes into account experimental cuts
was reported in Ref.~\cite{Anastasiou:2005qj}, in the case of the decay mode $H\to\gamma\gamma$.
In Ref.~\cite{Anastasiou:2007mz} the calculation is
extended to the decay mode $H\to WW\to l\nu l\nu$.

In Ref.~\cite{Catani:2007vq} we have presented an independent NNLO calculation
of the Higgs production cross section.
The method is completely different from
that used in Refs.~\cite{Anastasiou:2005qj,Anastasiou:2007mz}.
Our calculation is implemented
in a fully-exclusive parton level event generator.
This feature makes it particularly suitable for practical applications
to the computation of distributions in the form of bin histograms.
Our numerical program can be downloaded from \cite{hnnlo}.
The decay modes that are currently implemented
are $H\to \gamma\gamma$ and $H\to WW\to l\nu l\nu$.

In the following
we present a brief selection of results that can be obtained
by our program.
We consider Higgs boson production at the LHC and
use the MRST2004 parton distributions \cite{Martin:2004ir},
with parton densities and $\as$ evaluated at each corresponding order
(i.e., we use $(n+1)$-loop $\as$ at N$^n$LO, with $n=0,1,2$). The 
renormalization and factorization scales are fixed to the value 
$\mu_R=\mu_F=M_H$, where $M_H$ is the mass of the Higgs boson.

%\section{RESULTS FOR THE DECAY MODE $H\to \gamma\gamma$}
\subsection{Results for the Decay Mode $H\to\gamma\gamma$}
%==========================================
\begin{figure}
\begin{center}
\includegraphics[width=0.5\textwidth]{ptminmax}
 \caption{Distributions in $\ptmin$ and $\ptmax$ for the diphoton signal at the LHC. The cross section is divided by the branching ratio in two photons.}
\label{fig:isol}
\end{center}
\end{figure}
%==========================================

We consider the production of a Higgs boson of mass $M_H=125$ GeV in the
$H\to\gamma\gamma$ decay mode and follow
Ref.~\cite{CMStdr} to apply cuts on the photons.
For each event, we classify the photon transverse momenta according to their
minimum and maximum value,  
$\ptmin$ and $\ptmax$. The photons are required to be in the
central rapidity region, $|\eta|<2.5$, with  $\ptmin>35$~GeV
and $\ptmax>40$~GeV. We also require the photons to be isolated:
the hadronic (partonic) transverse energy in a cone of radius $R=0.3$ along the
photon direction 
has to be smaller than 6~GeV. By applying these cuts
the impact of the NNLO corrections on the NLO total cross section
is reduced from 19\% to 11\%.
 
In Fig.~\ref{fig:isol} we plot
the distributions in $\ptmin$ and $\ptmax$
of the signal process $gg\to H\to\gamma\gamma$.
We note that the shape of these distributions sizeably
differs when going from LO to NLO and to NNLO.
The origin of these perturbative instabilities is well known 
\cite{Catani:1997xc}.
Since the LO spectra
are kinematically bounded by $p_T\leq M_H/2$,
each higher-order perturbative contribution produces
(integrable) logarithmic singularities in the vicinity of
that boundary. More detailed studies are necessary to assess
the theoretical uncertainties of these fixed-order results
and the relevance of all-order resummed calculations.
 
In Fig.~\ref{fig:ctheta} we consider the (normalized) distribution in
the variable $\cos\theta^*$, where $\theta^*$ is the polar angle of one of the photons
in the rest frame of the Higgs boson
\footnote{We thank Suzanne Gascon and Markus Schumacher for suggesting
the use of this variable.}.
At small values of $\cos\theta^*$ the distribution
is quite stable with respect to higher order QCD corrections.
We also note that the LO distribution vanishes beyond the value $\cos\theta^*_{\rm max}<1$.
The upper bound $\cos\theta^*_{\rm max}$ is due to the fact that the photons
are required to have a minimum $p_T$ of $35$ GeV.
As in the case of Fig.~\ref{fig:isol}, in the vicinity of this LO kinematical boundary
there is an instability of the
perturbative results beyond LO.

%==========================================
\begin{figure}
\begin{center}
\includegraphics[width=0.5\textwidth]{cthetanew}
 \caption{Normalized distribution in the variable $\cos\theta^*$.}
\label{fig:ctheta}
\end{center}
\end{figure}
%==========================================

%\section{RESULTS FOR THE DECAY MODE $H\to l\nu l\nu$}
\subsection{Results for the Decay Mode $H\to l \nu l \nu$}
We now consider the production of a Higgs boson with mass $M_H=165$ GeV in the decay mode $H\to l\nu l\nu$.
We apply a set of preselection cuts taken from the study of Ref.~\cite{Davatz:2004zg}. The charged leptons have $p_T$ larger than 20 GeV, and $|\eta|<2$. The missing $p_T$ is
larger than $20$ GeV and the invariant mass of the charged
leptons is smaller than $80$ GeV.
Finally, the azimuthal separation of the charged leptons in the
transverse plane ($\Delta\phi$) is smaller than $135^o$.
By applying these cuts the impact of the NNLO corrections
on the NLO result does not change and is of about $20\%$.

%==========================================
\begin{figure}
\begin{center}
\includegraphics[width=0.5\textwidth]{deltaphinorm}
 \caption{Normalized $\Delta\phi$ distribution at LO, NLO, NNLO.}
\label{fig:deltaphi}
\end{center}
\end{figure}
%==========================================
In Fig.\ref{fig:deltaphi} we
plot the $\Delta\phi$ distribution at LO, NLO and NNLO.
As is well known \cite{Dittmar:1996ss},
the charged leptons from the Higgs boson
signal tend to be close in angle,
and thus the distribution is peaked at small $\Delta\phi$.
We notice that the effect of the QCD corrections is to increase
the steepness of the distribution,
from LO to NLO and from NLO to NNLO.

%\section{CONCLUSIONS}
\subsection{Conclusions}
We have illustrated a calculation of the Higgs boson production cross section at the LHC
up to NNLO in QCD perturbation theory. The calculation is implemented in the numerical program {\tt HNNLO},
which at present includes the decay modes $H\to\gamma\gamma$ and $H\to WW\to l\nu l\nu$. The program allows the user to apply arbitrary cuts on the momenta of the partons and leptons (photons) produced in the final state, and to obtain the required distributions in the form of
bin histograms. We have presented a brief selection of numerical results that
can be obtained by our program. The fortran code {\tt HNNLO} can be downloaded from \cite{hnnlo}.

%\bibliography{hnnlolh}
%
%\end{document}


==> paperdef.tex <==
\catcode`@=11
\def\citer{\@ifnextchar [{\@tempswatrue\@citexr}{\@tempswafalse\@citexr[]}}
 
\def\@citexr[#1]#2{\if@filesw\immediate\write\@auxout{\string\citation{#2}}\fi
  \def\@citea{}\@cite{\@for\@citeb:=#2\do
    {\@citea\def\@citea{--\penalty\@m}\@ifundefined
       {b@\@citeb}{{\bf ?}\@warning
       {Citation `\@citeb' on page \thepage \space undefined}}%
\hbox{\csname b@\@citeb\endcsname}}}{#1}}
\catcode`@=12

%\renewcommand{\topfraction}{1.0}
%\renewcommand{\bottomfraction}{0.3}
\renewcommand{\textfraction}{0}
\renewcommand{\floatpagefraction}{1.0}

% new commands for cross referencing
%\def\refeq#1{\mbox{(\ref{#1})}}
\def\refeq#1{\mbox{eq.~(\ref{#1})}}
\def\refeqs#1{\mbox{eqs.~(\ref{#1})}}
\def\reffi#1{\mbox{Fig.~\ref{#1}}}
\def\reffis#1{\mbox{Figs.~\ref{#1}}}
\def\refta#1{\mbox{Tab.~\ref{#1}}}
%\def\refta#1{\mbox{Table~\ref{#1}}}
\def\reftas#1{\mbox{Tabs.~\ref{#1}}}
%\def\reftas#1{\mbox{Tables~\ref{#1}}}
\def\refse#1{\mbox{Sect.~\ref{#1}}}
\def\refses#1{\mbox{Sects.~\ref{#1}}}
%\def\refse#1{\mbox{Section~\ref{#1}}}
\def\refapp#1{\mbox{App.~\ref{#1}}}
%\def\refapp#1{\mbox{Appendix~\ref{#1}}}
\def\citere#1{\mbox{Ref.~\cite{#1}}}
\def\citeres#1{\mbox{Refs.~\cite{#1}}}

\newcommand{\mst}{m_{\tilde{t}}}
\newcommand{\delmst}{\Delta\mst}
\newcommand{\mstr}{m_{\tilde{t}_R}}
\newcommand{\mstl}{m_{\tilde{t}_L}}
\newcommand{\mste}{m_{\tilde{t}_1}}
\newcommand{\mstz}{m_{\tilde{t}_2}}
\newcommand{\msti}{m_{\tilde{t}_i}}
\newcommand{\mstip}{m_{\tilde{t}_{i'}}}
\newcommand{\mstj}{m_{\tilde{t}_j}}
\newcommand{\msb}{m_{\tilde{b}}}
\newcommand{\msbr}{m_{\tilde{b}_R}}
\newcommand{\msbl}{m_{\tilde{b}_L}}
\newcommand{\msbe}{m_{\tilde{b}_1}}
\newcommand{\msbz}{m_{\tilde{b}_2}}
\newcommand{\msbi}{m_{\tilde{b}_i}}
\newcommand{\msbj}{m_{\tilde{b}_j}}
\newcommand{\MstL}{M_{\tilde{t}_L}}
\newcommand{\MstR}{M_{\tilde{t}_R}}
\newcommand{\MsbL}{M_{\tilde{b}_L}}
\newcommand{\MsbR}{M_{\tilde{b}_R}}
\newcommand{\MsqL}{M_{\tilde{q}_L}}
\newcommand{\MsqR}{M_{\tilde{q}_R}}
\newcommand{\Mtlr}{M_{t}^{LR}}
\newcommand{\Mtlrz}{\KL M_{t}^{LR}\KR^2}
\newcommand{\Mtlrd}{\KL M_{t}^{LR}\KR^3}
\newcommand{\Mtlrv}{\KL M_{t}^{LR}\KR^4}
\newcommand{\Mtlrf}{\KL M_{t}^{LR}\KR^5}
\newcommand{\Mtlrse}{\KL M_{t}^{LR}\KR^6}
\newcommand{\Mtlrsi}{\KL M_{t}^{LR}\KR^7}
\newcommand{\Mtlra}{\KL M_{t}^{LR}\KR^8}
\newcommand{\Mblr}{M_{b}^{LR}}
\newcommand{\Mblrz}{\KL M_{b}^{LR}\KR^2}
\newcommand{\Mqlr}{M_{q}^{LR}}
\newcommand{\At}{A_t}
\newcommand{\Ab}{A_b}
\newcommand{\Xt}{X_t}
\newcommand{\Xb}{X_b}
%\newcommand{\mot}{m_{1/2}}

\newcommand{\mstaue}{m_{\tilde{\tau}_1}}
\newcommand{\mstauz}{m_{\tilde{\tau}_2}}

\newcommand{\mf}{m_f}
\newcommand{\mfp}{m_{f'}}
\newcommand{\mfi}{m_{f_i}}
\newcommand{\msfr}{m_{\tilde{f}_R}}
\newcommand{\msfl}{m_{\tilde{f}_L}}
\newcommand{\msf}{m_{\tilde{f}}}
\newcommand{\msfi}{m_{\tilde{f}_i}}
\newcommand{\msfe}{m_{\tilde{f}_1}}
\newcommand{\msfz}{m_{\tilde{f}_2}}

\newcommand{\ms}{M_S}
\newcommand{\msusy}{M_{\rm SUSY}}
\newcommand{\msq}{m_{\tilde{q}}}
\newcommand{\msqi}{m_{\tilde{q}_i}}
\newcommand{\msqip}{m_{\tilde{q}_{i'}}}
\newcommand{\msqj}{m_{\tilde{q}_j}}
\newcommand{\msqe}{m_{\tilde{q}_1}}
\newcommand{\msqz}{m_{\tilde{q}_2}}

\newcommand{\sfn}{\tilde{f}}
\newcommand{\sfl}{\tilde{f}_L}
\newcommand{\sfr}{\tilde{f}_R}
\newcommand{\sfe}{\tilde{f}_1}
\newcommand{\sfz}{\tilde{f}_2}
\newcommand{\sfi}{\tilde{f}_i}
\newcommand{\sfj}{\tilde{f}_j}
\newcommand{\sfez}{\tilde{f}_{12}}
\newcommand{\sfze}{\tilde{f}_{21}}
\newcommand{\neone}{\tilde{\chi}^0_1}
\newcommand{\mneone}{m_{\tilde{\chi}^0_1}}
\newcommand{\netwo}{\tilde{\chi}^0_2}
\newcommand{\chone}{\tilde{\chi}^+_1}
\newcommand{\chonem}{\tilde{\chi}^-_1}
\newcommand{\chtwo}{\tilde{\chi}^+_2}
\newcommand{\chtwom}{\tilde{\chi}^-_2}


\newcommand{\Hi}{H_i}
\newcommand{\cHe}{\cH_1}
\newcommand{\cHz}{\cH_2}
\newcommand{\Pe}{\phi_1}
\newcommand{\Pz}{\phi_2}
\newcommand{\Pez}{\phi_{1,2}}
\newcommand{\PePz}{\phi_1\phi_2}
\newcommand{\mpe}{m_{\Pe}}
\newcommand{\mpz}{m_{\Pz}}
\newcommand{\mpez}{m_{\PePz}}

\newcommand{\smallz}{{\scriptscriptstyle Z}} %  a smaller Z
\newcommand{\smallD}{{\scriptscriptstyle D}} %
\newcommand{\smallQ}{{\scriptscriptstyle Q}} %
\newcommand{\smallU}{{\scriptscriptstyle U}} %

\newcommand{\SU}{\mathrm {SUSY}}
\newcommand{\SM}{\mathrm {SM}}
\newcommand{\hi}{\mathrm {Higgs}}
\def\Liz#1{{\rm Li}_2 \KL #1 \KR}
\newcommand{\msbar}{$\overline{\rm{MS}}$}
\newcommand{\msbarm}{\overline{\rm{MS}}}
\newcommand{\drbar}{$\overline{\rm{DR}}$}
\newcommand{\drbarm}{\overline{\rm{DR}}}
\newcommand{\oa}{{\cal O}(\alpha)}
\newcommand{\oas}{{\cal O}(\alpha_s)}
\newcommand{\oaas}{{\cal O}(\alpha\alpha_s)}
\newcommand{\ogmzmts}{{\cal O}(\gf^2\mt^6)}
\def\order#1{${\cal O}(#1)$}
\def\orderm#1{{\cal O}\KL #1 \KR}
\newcommand{\cp}{{\cal CP}}
\newcommand{\cA}{{\cal A}}
\newcommand{\cH}{{\cal H}}
\newcommand{\cHi}{{\cal H}_i}
\newcommand{\cL}{{\cal L}}
\newcommand{\cO}{{\cal O}}
\newcommand{\cZ}{{\cal Z}}
\newcommand{\wz}{\sqrt{2}}
\newcommand{\edz}{\frac{1}{2}}
\def\ed#1{\frac{1}{#1}}
\newcommand{\twol}{two-loop}
\newcommand{\onel}{one-loop}
\newcommand{\mma}{{\em Mathematica}}
\newcommand{\tc}{{\em TwoCalc}}
\newcommand{\fa}{{\em FeynArts}}
\newcommand{\fh}{{\em FeynHiggs}}
\newcommand{\fhf}{{\em FeynHiggsFast}}
\newcommand{\shp}{{\em subhpole}}
\newcommand{\rp}{$\rho\,$-parameter}

\newcommand{\MW}{M_W}
\newcommand{\MZ}{M_Z}
\newcommand{\MA}{M_A}
\newcommand{\mh}{m_h}
\newcommand{\mH}{m_H}
\newcommand{\Mh}{M_h}
\newcommand{\MH}{M_H}
\newcommand{\mhmax}{m_h^{\rm max}}
\newcommand{\mHp}{m_{H^\pm}}
\newcommand{\MHp}{M_{H^\pm}}
\newcommand{\mG}{m_G}
\newcommand{\mGp}{m_{G^\pm}}
\newcommand{\MHSM}{M_H^{\SM}}
\newcommand{\mhtree}{m_{h,{\rm tree}}}
\newcommand{\mHtree}{m_{H,{\rm tree}}}

\newcommand{\sudxsuzxue}{SU(3)_C \otimes SU(2)_L \otimes U(1)_Y}
\newcommand{\suzxue}{SU(2)_L \otimes U(1)_Y}

\newcommand{\dr}{\De\rho}
\newcommand{\mt}{m_{t}}
\newcommand{\Mt}{M_{t}}
\newcommand{\mtms}{\overline{m}_t}
\newcommand{\mq}{m_{q}}
\newcommand{\mb}{m_{b}}
\newcommand{\Mb}{M_{b}}
\newcommand{\db}{\De_b}
\newcommand{\mbms}{\overline{m}_b}
\newcommand{\gl}{\tilde{g}}
\newcommand{\Mgl}{m_{\tilde{g}}}
\newcommand{\mgl}{m_{\tilde{g}}}
\newcommand{\Sferm}{\tilde{f}}
\newcommand{\Sfermp}{\tilde{f}'}
\newcommand{\sq}{\tilde{q}}
\newcommand{\sqi}{\tilde{q}_i}
\newcommand{\sqj}{\tilde{q}_j}
\newcommand{\sql}{\tilde{q}_L}
\newcommand{\sqr}{\tilde{q}_R}
\newcommand{\sqe}{\tilde{q}_1}
\newcommand{\sqz}{\tilde{q}_2}
\newcommand{\sqez}{\tilde{q}_{12}}
\newcommand{\Stop}{\tilde{t}}
\newcommand{\StopL}{\tilde{t}_L}
\newcommand{\StopR}{\tilde{t}_R}
\newcommand{\Stope}{\tilde{t}_1}
\newcommand{\Stopz}{\tilde{t}_2}
\newcommand{\Stopi}{\tilde{t}_i}
\newcommand{\Stopj}{\tilde{t}_j}
\newcommand{\Sbot}{\tilde{b}}
\newcommand{\SbotL}{\tilde{b}_L}
\newcommand{\SbotR}{\tilde{b}_R}
\newcommand{\Sbote}{\tilde{b}_1}
\newcommand{\Sbotz}{\tilde{b}_2}
\newcommand{\Sboti}{\tilde{b}_i}
\newcommand{\Sbotj}{\tilde{b}_j}
\newcommand{\Stau}{\tilde{\tau}}
\newcommand{\Staue}{\tilde{\tau}_1}
\newcommand{\AStaue}{\bar{\tilde{\tau}}_1}
\newcommand{\Snet}{\tilde{\nu}_\tau}
\newcommand{\Smu}{\tilde \mu}
\newcommand{\Sneum}{\tilde \nu_\mu}
\newcommand{\dst}{\Delta_{\tilde{t}}}
\newcommand{\tst}{\theta_{\tilde{t}}}
\newcommand{\tsb}{\theta_{\tilde{b}}}
\newcommand{\tsf}{\theta\kern-.20em_{\tilde{f}}}
\newcommand{\tsfp}{\theta\kern-.20em_{\tilde{f}\prime}}
\newcommand{\tsq}{\theta\kern-.15em_{\tilde{q}}}
\newcommand{\sw}{s_W}
\newcommand{\cw}{c_W}
\newcommand{\sweff}{\sin^2\theta_{\mathrm{eff}}}
\newcommand{\aef}{a_{\rm eff}^f}
\newcommand{\vef}{v_{\rm eff}^f}

\newcommand{\cha}[1]{\tilde \chi^\pm_{#1}}
\newcommand{\mcha}[1]{m_{\tilde \chi^\pm_{#1}}}
\newcommand{\neu}[1]{\tilde \chi^0_{#1}}
\newcommand{\mneu}[1]{m_{\tilde \chi^0_{#1}}}

\newcommand{\sintt}{\sin\tst}
\newcommand{\sinQtt}{\sin^2\tst}
\newcommand{\sinZtt}{\sin 2\tst}
\newcommand{\sinQZtt}{\sin^2 2\tst}
\newcommand{\sintb}{\sin\tsb}
\newcommand{\sinQtb}{\sin^2\tsb}
\newcommand{\sinZtb}{\sin 2\tsb}
\newcommand{\sintf}{\sin\tsf}
\newcommand{\sintfp}{\sin\tsfp}
\newcommand{\sinQtf}{\sin^2\tsf}
\newcommand{\sinZtf}{\sin 2\tsf}
\newcommand{\sintq}{\sin\tsq}
\newcommand{\sinQtq}{\sin^2\tsq}
\newcommand{\sinZtq}{\sin 2\tsq}

\newcommand{\costt}{\cos\tst}
\newcommand{\cosQtt}{\cos^2\tst}
\newcommand{\cosZtt}{\cos 2\tst}
\newcommand{\costb}{\cos\tsb}
\newcommand{\cosQtb}{\cos^2\tsb}
\newcommand{\cosZtb}{\cos 2\tsb}
\newcommand{\costf}{\cos\tsf}
\newcommand{\costfp}{\cos\tsfp}
\newcommand{\cosQtf}{\cos^2\tsf}
\newcommand{\cosZtf}{\cos 2\tsf}
\newcommand{\costq}{\cos\tsq}
\newcommand{\cosQtq}{\cos^2\tsq}
\newcommand{\cosZtq}{\cos 2\tsq}

\newcommand{\stt}{s_{\tilde{t}}}
\newcommand{\stb}{s_{\tilde{b}}}
\newcommand{\stf}{s_{\tilde{f}}}
\newcommand{\stq}{s_{\tilde{q}}}
\newcommand{\ctt}{c_{\tilde{t}}}
\newcommand{\ctb}{c_{\tilde{b}}}
\newcommand{\ctf}{c_{\tilde{f}}}
\newcommand{\ctq}{c_{\tilde{q}}}

\newcommand{\KL}{\left(}
\newcommand{\KR}{\right)}
\newcommand{\KKL}{\left[}
\newcommand{\KKR}{\right]}
\newcommand{\KKKL}{\left\{}
\newcommand{\KKKR}{\right\}}
\newcommand{\BL}{\lbrack}
\newcommand{\BR}{\rbrack}

\newcommand{\VL}{\left( \begin{array}{c}}
\newcommand{\VR}{\end{array} \right)}
\newcommand{\ML}{\left( \begin{array}{cc}}
\newcommand{\MLd}{\left( \begin{array}{ccc}}
\newcommand{\MLv}{\left( \begin{array}{cccc}}
\newcommand{\MR}{\end{array} \right)}
\newcommand{\dd}{\partial}
\newcommand{\dmu}{\partial_{\mu}}
\newcommand{\dmo}{\partial^{\mu}}
\newcommand{\mn}{{\mu\nu}}
\newcommand{\hc}{\mbox {h.c.}}
\newcommand{\re}{\mbox {Re}\,}
\newcommand{\OP}{\omega_+}
\newcommand{\OM}{\omega_-}
\newcommand{\Tb}{\tan \beta\hspace{1mm}}
\newcommand{\tb}{\tan \beta}
\newcommand{\TQb}{\tan^2 \beta\hspace{1mm}}
\newcommand{\CTb}{\cot \beta\hspace{1mm}}
\newcommand{\CTQb}{\cot^2 \beta\hspace{1mm}}
\newcommand{\Sb}{\sin \beta\hspace{1mm}}
\newcommand{\sbe}{\sin \beta}
\newcommand{\SQb}{\sin^2\beta\hspace{1mm}}
\newcommand{\SDb}{\sin^3\beta\hspace{1mm}}
\newcommand{\SVb}{\sin^4\beta\hspace{1mm}}
\newcommand{\Cb}{\cos \beta\hspace{1mm}}
\newcommand{\CQb}{\cos^2\beta\hspace{1mm}}
\newcommand{\CDb}{\cos^3\beta\hspace{1mm}}
\newcommand{\CVb}{\cos^4\beta\hspace{1mm}}
\newcommand{\Sa}{\sin \alpha\hspace{1mm}}
\newcommand{\SQa}{\sin^2\alpha\hspace{1mm}}
\newcommand{\Ca}{\cos \alpha\hspace{1mm}}
\newcommand{\CQa}{\cos^2\alpha\hspace{1mm}}
\newcommand{\Ta}{\tan\al}
\newcommand{\CTa}{\cot\al}
\newcommand{\Sab}{\sin (\alpha + \beta)\hspace{1mm}}
\newcommand{\Cab}{\cos (\alpha + \beta)\hspace{1mm}}
\newcommand{\Sba}{\sin (\beta - \alpha)\hspace{1mm}}
\newcommand{\Samb}{\sin (\al - \be)\hspace{1mm}}
\newcommand{\Cba}{\cos (\beta - \alpha)\hspace{1mm}}
\newcommand{\Camb}{\cos (\al - \be)\hspace{1mm}}
\newcommand{\SZa}{\sin 2\alpha\hspace{1mm}}
\newcommand{\SQZa}{\sin^2 2\alpha\hspace{1mm}}
\newcommand{\CZa}{\cos 2\alpha\hspace{1mm}}
\newcommand{\CQZa}{\cos^2 2\alpha\hspace{1mm}}
\newcommand{\SZb}{\sin 2\beta\hspace{1mm}}
\newcommand{\SQZb}{\sin^2 2\beta\hspace{1mm}}
\newcommand{\CZb}{\cos 2\beta\hspace{1mm}}
\newcommand{\CQZb}{\cos^2 2\beta\hspace{1mm}}
\newcommand{\CDZb}{\cos^3 2\beta\hspace{1mm}}
\newcommand{\CVZb}{\cos^4 2\beta\hspace{1mm}}
\newcommand{\CQba}{\cos^2 (\beta - \alpha)\hspace{1mm}}
\newcommand{\SQba}{\sin^2 (\beta - \alpha)\hspace{1mm}}
\newcommand{\SDba}{\sin^3 (\beta - \alpha)\hspace{1mm}}
\newcommand{\CQab}{\cos^2 (\alpha + \beta)\hspace{1mm}}
\newcommand{\SQab}{\sin^2 (\alpha + \beta)\hspace{1mm}}
\newcommand{\SDab}{\sin^3 (\alpha + \beta)\hspace{1mm}}
\newcommand{\SDea}{\sin \De\al}
\newcommand{\CDea}{\cos \De\al}
\newcommand{\CQDea}{\cos^2\De\al}
\newcommand{\TDea}{\tan \De\al}
\newcommand{\TQDea}{\tan^2\De\al}

\newcommand{\tev}{\,\, \mathrm{TeV}}
\newcommand{\gev}{\,\, \mathrm{GeV}}
\newcommand{\mev}{\,\, \mathrm{MeV}}

\newcommand{\BC}{\begin{center}}
\newcommand{\EC}{\end{center}}
\newcommand{\BE}{\begin{equation}}
\newcommand{\EE}{\end{equation}}
\newcommand{\BEA}{\begin{eqnarray}}
\newcommand{\BEAnn}{\begin{eqnarray*}}
\newcommand{\EEA}{\end{eqnarray}}
\newcommand{\EEAnn}{\end{eqnarray*}}
\newcommand{\non}{\nonumber}
\newcommand{\id}{{\rm 1\kern-.12em
\rule{0.3pt}{1.5ex}\raisebox{0.0ex}{\rule{0.1em}{0.3pt}}}}
\newcommand{\lsim}
{\;\raisebox{-.3em}{$\stackrel{\displaystyle <}{\sim}$}\;}
%\newcommand{\gsim}
%{\;\raisebox{-.3em}{$\stackrel{\displaystyle >}{\sim}$}\;}


\newcommand{\cf}{C_F}
\newcommand{\gf}{G_F}
\newcommand{\Gf}{G_F}
\newcommand{\GF}{G_F}
\newcommand{\nf}{N_f}
% shorthands for greek letters
\def\al{\alpha}
\def\aeff{\al_{\rm eff}}
\def\aeffapprox{\al_{\rm eff}{\rm (approx)}}
\newcommand{\Saeff}{\sin\aeff}
\newcommand{\Caeff}{\cos\aeff}
\newcommand{\sbaeff}{\sin(\be-\aeff)}
\newcommand{\sqbaeff}{\sin^2(\be-\aeff)}
\def\als{\alpha_s}
\def\alt{\alpha_t}
\def\alb{\alpha_b}
\def\altl{\alpha_{\rm 2-loop}}
\def\gs{g_s}
\def\be{\beta}
\def\ben{\be_0}
\def\bee{\be_1}
\def\bez{\be_2}
\def\ga{\gamma}
\def\gan{\ga_0}
\def\gae{\ga_1}
\def\gaz{\ga_2}
\def\de{\delta}
\def\deqed{\de\Ga_\ga}
\def\eps{\varepsilon}
\def\la{\lambda}
\def\si{\sigma}
\def\ie{i\epsilon}
\def\om{\omega}
\def\ohsq{\Omega_\chi h^2}
\def\Ga{\Gamma}
\def\Gh{\Ga_h}
\def\GH{\Ga_H}
\def\Gz{\Ga_0}
\def\Ge{\Ga_1}
\def\Geeff{\Ga_{1,\rm eff}}
\def\Geg{\Ga_{1,g}}
\def\Gga{\Ga_\ga}
\def\Gg{\Ga_g}
\def\Ggl{\Ga_{\gl}}
\def\Gtot{\Ga_{\rm tot}}
\def\De{\Delta}
\def\La{\Lambda}
\def\Laqcd{\La_{\rm QCD}}
\def\Si{\Sigma}
\def\Sip{\Sigma'}
\def\Sie{\Sigma^{(1)}}
\def\Siz{\Sigma^{(2)}}
\def\Sii{\Sigma^{(i)}}
\def\Siep{\Sigma'^{(1)}}
\def\Sizp{\Sigma'^{(2)}}
\def\Siip{\Sigma'^{(i)}}

\def\hSi{\hat{\Sigma}}
\def\hSip{\hat{\Sigma}'}
\def\hSie{\hat{\Sigma}^{(1)}}
\def\hSiz{\hat{\Sigma}^{(2)}}
\def\hSiep{\hat{\Sigma}^{(1)}'}
\def\hSizp{\hat{\Sigma}^{(2)}'}
\def\hSiH{\hSi_{HH}}
\def\hSih{\hSi_{hh}}
\def\hSihH{\hSi_{hH}}
\def\hSipH{\hSip_{HH}}
\def\hSiph{\hSip_{hh}}
\def\hSiphH{\hSip_{hH}}
\def\hSieh{\hSie_{h}}
\def\hSieH{\hSie_{H}}
\def\hSiehH{\hSie_{hH}}
\def\hSizh{\hSiz_{h}}
\def\hSizH{\hSiz_{H}}
\def\hSizhH{\hSiz_{hH}}
\newcommand{\htad}{\hat{t}}
\newcommand{\tade}{t^{(1)}}
\newcommand{\tadz}{t^{(2)}}

\newcommand{\Ph}{\mathswitchr h}
\newcommand{\PH}{\mathswitchr H}

\newcommand{\deMZe}{\de \MZ^{2\,(1)}}
\newcommand{\deMZz}{\de \MZ^{2\,(2)}}
\newcommand{\deMZi}{\de \MZ^{2\,(i)}}
\newcommand{\deMAe}{\de \MA^{2\,(1)}}
\newcommand{\deMAz}{\de \MA^{2\,(2)}}
\newcommand{\deMAi}{\de \MA^{2\,(i)}}
\newcommand{\deZHie}{\de Z_{H_i}^{(1)}}
\newcommand{\deZHiz}{\de Z_{H_i}^{(2)}}
\newcommand{\deZHee}{\de Z_{H_1}^{(1)}}
\newcommand{\deZHez}{\de Z_{H_1}^{(2)}}
\newcommand{\deZHze}{\de Z_{H_2}^{(1)}}
\newcommand{\deZHzz}{\de Z_{H_2}^{(2)}}
\newcommand{\deTbe}{\de\Tb^{(1)}}
\newcommand{\deTbz}{\de\Tb^{(2)}}
\newcommand{\detie}{\de t_i^{(1)}}
\newcommand{\detiz}{\de t_i^{(2)}}
\newcommand{\detee}{\de t_1^{(1)}}
\newcommand{\detez}{\de t_1^{(2)}}
\newcommand{\detei}{\de t_1^{(i)}}
\newcommand{\detze}{\de t_2^{(1)}}
\newcommand{\detzz}{\de t_2^{(2)}}
\newcommand{\detzi}{\de t_2^{(i)}}
\newcommand{\deVie}{\de V_i^{(1)}}
\newcommand{\deViz}{\de V_i^{(2)}}
\newcommand{\deVee}{\de V_{\Pe}^{(1)}}
\newcommand{\deVez}{\de V_{\Pe}^{(2)}}
\newcommand{\deVei}{\de V_{\Pe}^{(i)}}
\newcommand{\deVze}{\de V_{\Pz}^{(1)}}
\newcommand{\deVzz}{\de V_{\Pz}^{(2)}}
\newcommand{\deVzi}{\de V_{\Pz}^{(i)}}
\newcommand{\deVeze}{\de V_{\PePz}^{(1)}}
\newcommand{\deVezz}{\de V_{\PePz}^{(2)}}
\newcommand{\deVezi}{\de V_{\PePz}^{(i)}}


\newcommand{\SLASH}[2]{\makebox[#2ex][l]{$#1$}/}
\newcommand{\Dslash}{\SLASH{D}{.5}\,}
\newcommand{\dslash}{\SLASH{\dd}{.15}}
\newcommand{\kslash}{\SLASH{k}{.15}}
\newcommand{\pslash}{\SLASH{p}{.2}}
\newcommand{\qslash}{\SLASH{q}{.08}}

\newcommand{\sqmsmt}{\sqrt{\ms^2-\mt^2}}
\newcommand{\sqmsmtbar}{\sqrt{\ms^2-\mtms^2}}
\newcommand{\lmtms}{\KL\frac{\mt^2}{\ms^2}\KR}
\newcommand{\lmtmsms}{\KL\frac{\mtms^2}{\ms^2}\KR}
\newcommand{\lmsmt}{\KL\frac{\ms^2 - \mt^2}{\mt^2}\KR}

\newcommand{\lc}{linear collider}
\newcommand{\epem}{$e^+e^-$}
\newcommand{\eetohZhA}{$e^+e^- \to hZ,hA$}
\newcommand{\eetohZ}{$e^+e^- \to hZ$}
\newcommand{\eetohA}{$e^+e^- \to hA$}
\newcommand{\ipb}{$\mbox{pb}^{-1}$}
\newcommand{\ifb}{$\mbox{fb}^{-1}$}
\newcommand{\iab}{$\mbox{ab}^{-1}$}
\newcommand{\gvf}{g_V^f}
\newcommand{\gaf}{g_A^f}
\newcommand{\AFB}{A_{\rm FB}}
\newcommand{\ALR}{A_{\rm LR}}

%\newcommand{\plane}[2]{$#1$--$#2$~plane}
\newcommand{\plane}[2]{($#1, #2$)~plane}

\newcommand{\br}{{\rm BR}}
\newcommand{\hff}{h \to f\bar{f}}
\newcommand{\Hff}{H \to f\bar{f}}
\newcommand{\hbb}{h \to b\bar{b}}
\newcommand{\Hbb}{H \to b\bar{b}}
\newcommand{\htautau}{h \to \tau^+\tau^-}
\newcommand{\hcc}{h \to c\bar{c}}
\newcommand{\rf}{R_f}
\newcommand{\hmumu}{h \to \mu^+\mu^-}
\newcommand{\mumuh}{\mu^+ \mu^- \to h}
\newcommand{\hWW}{h \to WW^*}
\newcommand{\WWh}{WW \to h}
\newcommand{\WWH}{WW \to H}
\newcommand{\hgg}{h \to gg}
\newcommand{\hgaga}{h \to \ga\ga}
\newcommand{\gagah}{\ga \ga \to h}
\newcommand{\staustauH}{\Staue\AStaue \to H}
%\newcommand{\cff}{C_{ff}}
\newcommand{\cff}{C_f^{(u)}}
%\newcommand{\cfpfp}{C_{f'f'}}
\newcommand{\cfpfp}{C_f^{(d)}}
\newcommand{\Zh}{Z_h}
\newcommand{\wZh}{\sqrt{\Zh}}
\newcommand{\ZH}{Z_H}
\newcommand{\wZH}{\sqrt{\ZH}}
\newcommand{\ZhH}{Z_{hH}}
\newcommand{\ZHh}{Z_{Hh}}
\newcommand{\Zext}{\cZ^{\rm ext}}
\newcommand{\Zmix}{\cZ^{\rm mix}}
\newcommand{\rS}{{\rm S\,}}
\newcommand{\rP}{{\rm P\,}}
\def\ul#1{\underline{\vphantom{g}#1}}

\newcommand{\amu}{a_\mu}
\newcommand{\amuX}{a_\mu^{\chi,{\rm 2L}}}
\newcommand{\amuSUoL}{a_\mu^{\rm SUSY,1L}}
\newcommand{\amuexp}{a_\mu^{\rm exp}}
\newcommand{\amutheo}{a_\mu^{\rm theo}}
\newcommand{\amuMSSM}{a_\mu^{\rm MSSM}}
\newcommand{\amuMSSMtl}{a_\mu^{\rm MSSM, 2L}}
\newcommand{\amuSUbos}{a_\mu^{\rm bos,2L, MSSM}}
\newcommand{\SUbos}{{\rm bos,2L, MSSM}}
\newcommand{\delamu}{\De\amu^{\rm 2L}}

\newcommand{\mpar}[1]{\marginpar{\tiny #1}}
\def\mua{\marginpar[\boldmath\hfil$\uparrow$]%
                   {\boldmath$\uparrow$\hfil}%
                    \typeout{marginpar: $\uparrow$}\ignorespaces}
\def\mda{\marginpar[\boldmath\hfil$\downarrow$]%
                   {\boldmath$\downarrow$\hfil}%
                    \typeout{marginpar: $\downarrow$}\ignorespaces}
\def\mla{\marginpar[\boldmath\hfil$\rightarrow$]%
                   {\boldmath$\leftarrow $\hfil}%
                    \typeout{marginpar: $\leftrightarrow$}\ignorespaces}
\def\Mua{\marginpar[\boldmath\hfil$\Uparrow$]%
                   {\boldmath$\Uparrow$\hfil}%
                    \typeout{marginpar: $\Uparrow$}\ignorespaces}
\def\Mda{\marginpar[\boldmath\hfil$\Downarrow$]%
                   {\boldmath$\Downarrow$\hfil}%
                    \typeout{marginpar: $\Downarrow$}\ignorespaces}
\def\Mla{\marginpar[\boldmath\hfil$\Rightarrow$]%
                   {\boldmath$\Leftarrow $\hfil}%
                    \typeout{marginpar: $\Leftrightarrow$}\ignorespaces}
\newcommand{\todo}[1]{\mbox{}\\ {\bf XXXXXXXXXXXXXXXXXXXXXXXXXXXXXXX}\\
                      {\bf #1}\\{\bf XXXXXXXXXXXXXXXXXXXXXXXXXXXXXXX}\\
                      \mbox{}\\}                 

\newcommand{\Atwo}{{\bf P3}}
\newcommand{\Athree}{{\bf P1}}
\newcommand{\Afour}{{\bf P4}}
\newcommand{\Afive}{{\bf P2}}


